Causal Data Integration

Causal inference is fundamental to empirical scientific discoveries in natural and social sciences; however, in the process of conducting causal inference, data management problems can lead to false discoveries. Two such problems are (i) not having all attributes required for analysis, and (ii) misidentifying which attributes are to be included in the analysis. Analysts often only have access to partial data, and they critically rely on (often unavailable or incomplete) domain knowledge to identify attributes to include for analysis, which is often given in the form of a causal DAG. We argue that data management techniques can surmount both of these challenges. In this work, we introduce the Causal Data Integration (CDI) problem, in which unobserved attributes are mined from external sources and a corresponding causal DAG is automatically built. We identify key challenges and research opportunities in designing a CDI system, and present a system architecture for solving the CDI problem. Our preliminary experimental results demonstrate that solving CDI is achievable and pave the way for future research.

==> opportunities.tex <==
\vspace{-2mm}
\subsection{Opportunities \& Limitations}
\label{subsec:limitations}

Despite the fact our preliminary experiments showed promising
results, there are still many future opportunities.\\
\noindent
\textit{\textbf{O1. Unstructured Data}}: Another source of possible latent factors is unstructured data such as text documents and images. Previous work demonstrated the advantages of representation learning techniques for feature generation to improve prediction models~\cite{bengio2013representation} and detect unobserved confounding variables~\cite{zeng2022uncovering}. Future work could develop methods for extracting interpretable features from unstructured data sources tailored for causal inference. \brit{Babak, please add more details here} \\
\textit{\textbf{O2. Human-in-the-Loop}}: Text-mining causal discovery algorithms, as well as generative models (e.g., GPT-3 \cite{brown2020language}), cannot be fully trusted. 
Achieving high
accuracy in determining causal relationships is still a
challenge for CDI; it requires substantial in-domain knowledge. Hence, a possible improvement is to use human-in-the-loop tasks, minimizing human effort while maximizing accuracy. \\ 
\textit{\textbf{O3. The C-DAG Problem}}: \common{Our best-effort algorithm does not ensure that the right adjustment set of attributes is identifiable from the output C-DAG. An interesting future work is to study the computational complexity of the C-DAG problem, and to devise an efficient algorithm with theoretical guarantees to solve it. 
While there is a rich body of work on graph summarization~\cite{zhang2010discovery,tian2008efficient,kumar2018utility,ko2020incremental}, we believe that a tailored causal solution is required. Another interesting open question is whether a single C-DAG is sufficient for a set of causal questions with different exposure and outcome attributes. Future research will examine if it is reasonable to expect that a single C-DAG is adequate to identify the correct adjustment sets of multiple causal questions.}   




==> related.tex <==
\section{Related work}
\label{sec:related}


\textbf{Data Integration}: 
Data integration focuses on combining data from different sources % and making it useful for data consumers,  
and provides a range of methods that can gather useful attributes for a CDI system.
Such methods enable a CDI system to extend input tables with entities from Knowledge Graphs (KGs)~\cite{parravicini2019fast} and with tables from data lakes~\cite{zhang2020finding, nargesian2018table}.
% A CDI system can be built upon, and even extend, existing data integration tools.
However, the CDI task sets itself apart from the classical data integration task
in their goals: data integration provides a \textit{materialized table view} on an underlying \textit{federated database} for \textit{general data analysis}, whereas CDI provides a \textit{graph view} on the underlying \textit{causal DAG} for \textit{causal analysis}. These different goals entail distinct measures of success; the success of a data integration system is defined by its ability to tie tuples from different sources, whereas the success of a CDI system is defined by its ability to discover relevant unobserved variables and recover the correct adjustment set of variables. 

%\noindent
% \textbf{Data Discovery}:
% \revised{We can rely on the rich body of work on data discovery methods \cite{bogatu2020dataset,castelo2021auctus} to find
% relevant data sources that can be aligned with
% the input table. However, existing methods use notions of relevance for discovery, whereas we aim to find unobserved confounding variables relevant to cause-effect estimations.
% Recent work proposed solutions which, when given an input table and a target column, discover joinable datasets with column(s) correlated with the target column~\cite{esmailoghli2021cocoa,santos2021correlation}. Such techniques can be used for
% extracting candidate confounding attributes from tabular data. }

% Recent work proposed solutions to discover datasets that can be joined with an input table and contain a column that is correlated with a target column~\cite{esmailoghli2021cocoa,santos2021correlation}.
% Such techniques can be used for
% extracting candidate confounding attributes from tabular data. However, confounding attributes affect not only the outcome but also the exposure, which is out of the scope of the current
% solutions.
% \anna{i don't feel like i understand this segment; current solutions don't account for how confounding attributes also affect the exposure variables? and how does this idea tie back to relating this body of work with our work?}
% Thus, future work will extend these techniques to support our goal.}





\noindent
\textbf{Pattern Recognition and Prediction}: 
Pattern recognition and 
prediction techniques, which aim to predict outcomes based on patterns in the data, are commonly used by researchers to make sense of the world.
Such methods are based in recognizing associations between variables, which
are not designed to determine cause-effect relations between correlated variables \cite{sharma2020causal},
are vulnerable to confounding bias, where
uncontrolled confounding variables
may cause spurious associations between features and outcomes \cite{pearl2018book}.
Causal inference techniques enable analysts to overcome such challenges when discerning the effects of interventions. 
While some ML methods can predict the effects of interventions
if provided with causal background knowledge
\cite{guo2021survey}, %,yao2021survey
such knowledge is challenging and costly to provide \cite{glymour2019review}.
A CDI system aims to
automatically build a high-fidelity causal graph to enable causal inference with any statistical or ML technique a user wishes to use.

% \textbf{Explainable AI}: 
% A related line of work is Explainable AI (XAI), an emerging field in ML that aims to address how black box decisions of AI systems are made. 
% XAI systems enable analysts to gain causal reasoning for model decisions \cite{chou2022counterfactuals}. Posthoc XAI systems allow analysts to decipher trained, black-box models, providing approximations (often based on correlations between features) to
% predictive models that do not necessarily match their true underlying mechanisms~\cite{rudin2019stop}. Other XAI systems explain which changes to the features would be necessary to accomplish the desired prediction~\cite{verma2020counterfactual}. While XAI systems aim to answer causal questions about the behavior of a model, CDI assists analysts in answering causal questions about the mechanisms of real-world processes by mining unobserved variables and the underlying causal DAG. 







\noindent
\textbf{Causal Discovery}:
\label{subsec:causal_discovery}
Causal discovery is a well-studied problem~\cite{glymour2019review}, whose goal is to infer causal relations among a set of attributes. Existing solutions can be split into two main approaches.
Data-centric methods infer a causal DAG based on data properties~\cite{glymour2019review}.
Though it is well-known that background knowledge is required to determine causal relations~\cite{pearl2018book}, 
a causal DAG can be inferred from the data
under some assumptions %kalainathan2018structural,
\cite{glymour2019review,chickering2002optimal} (e.g.,
sufficiency,
faithfulness). % and generation process
Prominent methods include constraint-based algorithms (e.g., PC, FCI \cite{spirtes2000causation}) and score-based algorithms (e.g., LiNGAM \cite{shimizu2006linear}, GES \cite{chickering2002optimal}, including ML approaches \cite{wiering2002evolving,zhu2019causal}).
However, such assumptions
may not hold in practice, and therefore limit the applicability of these algorithms.
Further, such algorithms may not capture causal relations that are not present in the data,
and ignore semantic and contextual information found in the attribute names and values.


Text-mining approaches infer causal relations among concepts by extracting claims of causal relationships from text documents. 
Methods for extracting causal relations from Wikipedia were presented in~\cite{hashimoto2019weakly,heindorf2020causenet}, and a method for causal relations mining from news articles was presented in \cite{hassanzadeh2019answering}. 
A promising model that has been trained to discover causal relations is
GPT-3~\cite{brown2020language}, a language model
that is applied without gradient updates or fine-tuning, 
via text interaction with the model. 
The strength of such methods is in identifying cause-effect relations between seemingly-independent attributes or relations that otherwise could not be found in the data.
However, they may fail to distinguish between direct and indirect effects, resulting in graphs containing redundant edges.
Further, such methods are also sensitive to the quality of attribute names. 

We propose a hybrid approach the merges the two approaches, to overcome their shortcomings and benefit from their advantages. 




% \anna{make reference to how this section is now after the intro and before the system sections; move content as necessary}
% \mike{answer the question people will inevitably have: why not just train an ML classifier and move on?}
% \brit{you can use ML for causal reasoning}
% \brit{talk about ML - they can be used to causal reasoning}
% \brit{pearl model is the best to answer causal questions}
% \mike{people do use methods based in ML; answering questions... causal reasoning -- pearl is most successful so far. causal questions vs. causal reasoning. we're not saying pearl model is best, but best design decision. can't say ML models won't work; regression weights help causal interpretations, but pearl model is the best approach to answer causal questions}
% \anna{
% % shapley values -- which features contribute most to the prediction, 'explainable ai'... the feature is likely to be causally related to the prediction. asking a question about causal behavior in prediction, not about underlying causal mechanisms in the data... causal inference is important... the most popular framework is the pearl framework which we adapt in this work

% % ML is great, especially for prediction

% prediction tasks rock, and ML classifiers have been successful
% however, sometimes predictions cannot answer causal questions
% \cite{yao2021survey,guo2021survey}
% (1) association ~ causality (association is not causality)
% -> ". The lowest level, Association (seeing/observing), entails the sensing of regularities or patterns in the input data, expressed as correlations. The middle level, Intervention (doing), predicts the effects of deliberate actions, expressed as causal relationships. The highest level, Counterfactuals (imagining), involves constructing a theory of (part of) the world that explains why specific actions have specific effects and what happens in the absence of such actions."
% (2) looking at features makes you vulnerable for confounding vars -- 'confounding bias'
% when you do prediction, follow attributes, confounding bias is not even a concern -- they're concerned with accuracy of prediction
% in causal inference, the goal is to find a model that aligns with the real world underlying mechanism
% ML models need to understand causality for them to avoid these pitfalls \cite{yao2021survey, guo2021survey}
% they are doing something else, counterfactual questions analyzing features in xai
% -> explainable ai / shapley values focus on features which contribute most to the prediction, causal mechanisms to explain an associative/predictive model with strong iid assumptions "asking a question about causal behavior in prediction, not about underlying causal mechanisms in the data"


% % we have causal inference to estimate causal effect (below)
% % the most popular framework is pearl's which we adapt in this work % didn't mention potential outcome model
% % -> restated, causal reasoning -- pearl is a dominant, popular framework which we adapt in this work
% % Causal inference enables analysts to answer different types of queries about \emph{direct, total and indirect causal effects} \cite{pearl2000models} and investigate causal relationships between independent and dependent 
% % variables from a dataset. In this work, we adapted the commonly used Pearls' causal inference approach \cite{pearl2000models}.

% }
% \brit{in the related work, when talking about ML, you can say something like: ". The lowest level, Association (seeing/observing), entails the sensing of regularities or patterns in the input data, expressed as correlations. The middle level, Intervention (doing), predicts the effects of deliberate actions, expressed as causal relationships. The highest level, Counterfactuals (imagining), involves constructing a theory of (part of) the world that explains why specific actions have specific effects and what happens in the absence of such actions."}
% \anna{
% actual causal inference ML based models...
% and the standard ML methods people know and love
% }
%
% causal questions
% explainable ai / shapley values focus on features which contribute most to the prediction, causal mechanisms to explain an associative/predictive model with strong iid assumptions "asking a question about causal behavior in prediction, not about underlying causal mechanisms in the data"
% causal reasoning -- pearl is a dominant, popular framework which we adapt in this work
%











% , such as news articles \cite{hassanzadeh2019answering}, Wikipedia articles \cite{hashimoto2019weakly,heindorf2020causenet}, and text crawled from the Web \cite{brown2020language}.

% , which do not always hold in practice.
% In addition,
% some score-based causal discovery
% algorithms make
% further assumptions
% % certain distributional assumptions, and LiNGAM further requires assumptions
% about
% attribute distributions,
% the data generation process, and lack of unobserved confounders \cite{chickering2002optimal, shimizu2006linear}; 



% \anna{babak said: 'Then mention there is an line of work in AI and ML dedicated to discovery of causal DAG from data and mention there restrictions (they can only discover a causal of dags, need a lot of data, intractable, ...) so they can not be relied on for and end-to-end causal analysis.' PC etc. have the 'as dataset gets big' expectation. running time depends on attributes or something? perhaps ask babak about intractable? what did you mean that causal dag algorithms are intractable?
% in poc, don't have to describe the algorithms, just mention them and cite them, but don't explain anything
% need to identify sufficient conditions for the output to be a dag
% pc / fci produce a class of DAGs and make it hard to do causal inference (pending convo with brit to clarify) "generally, that means that the DAGs can not be fully relied on for an end-to-end causal analysis"
% require a lot of data -- sensitive to measurement error and selection bias \cite{glymour2019review}
% "For what Babak said about the need for a lot of data, please look on the Lingam and GES papers to see how big were their datasets in the experiments. If all datasets are relatively big, this is good enough"
% }
% However, such methods can only discover a class of causal DAGs, are highly sensitive to selection bias, and often use assumptions that may not hold in practice \cite{glymour2019review}. Thus, such methods can not be fully relied on for an end-to-end causal analysis.




% infer causal relations based on properties of the input dataset (e.g., conditional independencies between attributes), assuming that key assumptions are held.
% Some of these assumptions include:
% \cite{kalainathan2018structural, glymour2019review}:
% sufficiency (there are no unobserved confounders);
% faithfulness (the graph implies all conditional independence relations between the variables); and
% the Markov property (every variable is independent of its non-descendants, given its parents); 
%and
%the DAG assumption (the causal graph is a directed acyclic graph).
% Notable examples of such solutions include
% Such data-centric causal discovery methods

% (such as the Peter-Clark (PC) algorithm \cite{spirtes2000causation} and the Fast Causal Inference (FCI) algorithm \cite{spirtes2000causation})
% where causal relationships are determined through reasoning about conditional independencies drawn from the data,

% (such as Greedy Equivalence Search (GES) \cite{chickering2002optimal} and the Linear,
% Non-Gaussian, Acyclic Model (LiNGAM) algorithm \cite{shimizu2006linear})
% maximizes the likelihood of the dataset existing if the causal graph accurately reflects the true causal graph \cite{glymour2019review}.





==> response.tex <==
\twocolumn

\section*{Response to the Reviewers}
\noindent \textbf{Dear reviewers,}

\noindent 
We would like to express our gratitude to the reviewers for their valuable feedback, which helped us improve our paper.
In response to the reviewers' comments, we focused on addressing four main areas of improvement:
(1) Adding a running 
example to highlight the challenges and opportunities of a CDI system;
(2) Clarification of the relationship between existing DB concepts and causal inference;
(3) Extending the discussion on robustness, and
(4) Expanding the discussion of opportunities and limitations.
To address these issues, we have provided a detailed explanation of our responses to the main concerns that were raised by all reviewers. We have also addressed each reviewer's comments individually.




\vspace{1mm}
\noindent
{\bf{(\colorbox{pink}{Point \textrm{1}}) Running Example}}. Following the reviewers' suggestion, we have expanded our running example from the Introduction to illustrate the challenges and opportunities of a CDI system better. Here, we summarize the main changes we made:

First, we revised the example in the Introduction to illustrate the input dataset (see Table \ref{tab:example}). Second, in Section \ref{sec:problem}, we now present a causal DAG depicting the causal relationships for our running example input dataset (see Figure \ref{fig:c_dag}). We further revised Example \ref{ex:causal_dag} to illustrate the role of the causal DAG in identifying the correct adjustment set for a given cause-effect estimation.   

Further, for each subsection in Section \ref{sec:system} describing one of the system components, we added an example explaining how it operates. Specifically, in Example \ref{ex:knowledge_extractor}, we illustrate how the \emph{Knowledge Extractor} extracts unobserved attributes from the US Open data lake by joining the input dataset with a table containing statistics on population size (based on state names). From DBpedia, it extracts multiple available properties of each state (by aligning the state name with its unique entity in DBpedia), including attributes describing the weather (e.g., min/avg temperature and amount of snow) and current governor. A visualization of the extracted attributes is given in Table \ref{tab:extracted_att}. In Example \ref{ex:data_org}, we discuss how the \emph{Data Organizer} handles functional dependencies and missing values, and in Example \ref{ex:causal_dag_builder}, we discuss how the \emph{Causal DAG Builder} construct a clustered causal DAG for the augmented dataset. A visualization of the generated clustered causal DAG is given in Figure \ref{fig:c_dag}. 



\vspace{1mm}
\noindent
{\bf{(\colorbox{pink}{Point \textrm{2}}) Relationship Between DB Concepts and Causal Inference}}. Our revised paper discusses the connection between two common DB concepts and causal inference. 

We added the following text to Section \ref{subsec:knowledgeextraction} to discuss the connection between the \emph{unconfoundedness assumption} in causal inference and the \emph{closed-world assumption} in databases: 



\textsf{The primary goal of the \emph{Knowledge Extractor} is to extract all relevant variables from the provided data sources to enable reliable and interpretable causal inference. In causal inference, the \emph{unconfoundedness assumption}~\cite{pearl2009causal} (the assumption that all the variables affecting both the exposure $T$ and the outcome $Y$ are observed and can be controlled for) is a key consideration. This assumption is similar to the closed-world assumption in database in that it assumes that the whole database is complete. However, since complete knowledge of all variables that affect both $T$ and $O$ is often unattainable, the focus should be on extracting all relevant variables from the provided data sources. The module is designed to ensure that as much relevant information as possible can be automatically extracted from the provided data sources, and its capabilities can be expanded over time to incorporate new sources or refine the extraction and integration process.}



Further, we added the following text to revised Section \ref{subsec:data_organizer} to explain the relationship between logical dependencies and the \emph{strict positivity assumption} in causal inference: 


\textsf{We search for attributes affecting both the exposure $T$ and the outcome $O$. The presence of logical dependencies can hinder this process, as they can obscure the true relationships between them. In particular, the causal inference literature assumes that the underlying distribution is \emph{strictly positive}~\cite{pearl2000models}. 
% meaning that all events have a non-zero probability
This assumption breaks down in the presence of logical dependencies: Assume we have an attribute $E$ with the functional dependency $E {\Rightarrow} T$. This means that when conditioning on $E$, there is no association between $T$ and $O$, 
regardless of the choice of $O$ and the causal relationship between $T$ and $O$. Namely, the existence of such an attribute $E$ violates the strict positivity assumption. 
Thus, we must handle attributes with functional dependencies with $T$ or $O$. A straightforward solution is to discard such attributes~\cite{salimi2018bias}. Another possible solution is to group attributes with functional dependencies, treating them as a single node in the causal DAG. We plan to develop a principled approach to discovering causal relations with the presence of functional dependencies.}


\vspace{1mm}
\noindent
{\bf{(\colorbox{pink}{Point \textrm{3}}) Robustness}}. Following the reviewers' advice, we extended the discussion about the robustness of the system; % . Specifically, in the robustness definition, we now include, besides 
beyond missing values, we also include other data quality issues (such as functional dependencies or data duplication) that may hinder the validity of the resulting causal analysis.


In Section \ref{subsec:challenges}, we revised the text regarding the challenge of robustness as follows: 

\textsf{The robustness of a CDI system is determined by its ability to handle various data quality issues that may arise during the data integration process. As in general data integration, there are multiple data quality issues that a CDI system has to face, including missing values and outliers. 
The impact of such data quality issues on causal inference is particularly significant. Unlike in traditional machine learning, where data quality issues may only result in a slight drop in accuracy, these issues can lead to false discoveries and erroneous conclusions in causal inference if not handled properly. This is because if these issues are not randomly distributed across different exposure groups, they can significantly impact the validity of the resulting conclusions. One common data quality issue that can significantly impact causal inference is missing data. Extracted attributes may contain missing values, which can lead to selection bias and erroneous conclusions. Thus, a key challenge is to ensure that the system is robust to---and effectively handles ---various data quality issues
to ensure the validity of the resulting causal analysis.}


 % }


In Section \ref{subsec:data_organizer}, we added the following text: 

\textsf{The \emph{Data Organizer} receives the extracted attributes and outputs a single augmented dataset. Extracted attributes may
contain data quality issues, such as missing values and data duplication, which can compromise the reliability of causal analysis. A successful implementation of
this module would handle all data quality issues and ensure that the system is robust to data quality issues.} 

Last, when discussing the challenges and opportunities of the \emph{Data Organizer} module, we added the following text: 

\textsf{Other data quality issues, such as inconsistencies, duplicates, and outliers, can also compromise the reliability of causal inference and lead to false discoveries and erroneous conclusions, if not handled properly. This is because if these issues are not randomly distributed across the exposure groups, they can lead to bias that may significantly impact the validity of the resulting conclusions. Using existing data-cleaning techniques (e.g., \cite{chu2016data,ilyas2019data}) may not be sufficient to address these issues in the context of causal inference, as they are not designed to validate that bias is resolved. As a result, there is a need for innovative techniques that can effectively address these data quality issues to ensure accurate and reliable causal analysis. This is particularly important in high-stakes domains, such as healthcare, where erroneous conclusions can have severe consequences for patients and healthcare providers.}



\vspace{1mm}
\noindent
{\bf{(\colorbox{pink}{Point \textrm{4}}) Opportunities and Limitations}}. Following the reviewers' comments, throughout the paper, we have extended the discussion about the challenges and opportunities of CDI. We further defer the description of our initial solutions to Section \ref{sec:poc} to better distinguish between the challenges and proposed solutions.  


Specifically, we added the following text to Section \ref{sec:intro}: 

\textsf{The first challenge is to augment an input dataset with unobserved variables, ensuring the \emph{output causal DAG is complete} (i.e., there are no unobserved confounding variables). 
Data discovery methods have been extensively researched to identify relevant data sources that can be integrated with an input dataset for attribute extraction~\cite{bogatu2020dataset,castelo2021auctus}. However, these methods are not specifically designed to discover unobserved attributes that are relevant for cause-effect estimation. This presents a unique opportunity to develop dedicated data discovery tools tailored for identifying unobserved confounding variables.}


\textsf{Extracted attributes may contain data quality issues, such as outliers and missing values. These issues may lead to erroneous conclusions, compromising the reliability of causal inference. In particular, missing values pose a significant challenge in causal inference as they may result in \emph{selection bias}~\cite{bareinboim2012controlling}, where certain samples are preferentially excluded from the data. Other data quality issues, such as inconsistent data formats and data duplication, can also impact the accuracy of causal inference analysis. Therefore, in addition to handling missing values, it is crucial to ensure that the system is robust to various data quality issues to ensure the validity of causal inference results.}



\textsf{The challenge of identifying the correct adjustment set of confounders\footnote{In causal inference, identifiability typically refers to the conditions that permit measuring causal effect from observed data. Here, we discuss the ability to identify a sufficient adjustment set of variables for accurate causal inference.} and constructing a causal DAG is particularly difficult when dealing with hundreds of extracted attributes. A human-driven causal DAG construction (from background knowledge and domain expertise) is infeasible in this scenario, and automatic methods for building a full causal DAG over all attributes may not be feasible either~\cite{glymour2019review}. To this end, we propose the construction of a cluster causal DAG (C-DAG)~\cite{anand2022effect}, which groups related attributes and only specifies the causal relationships between clusters of attributes. By doing so, the correct adjustment set of attributes can still be identifiable from this C-DAG. This approach reduces cognitive overhead for analysts and makes causal analysis possible for high-dimensional data, which is currently not feasible for existing tools (e.g., \cite{sharma2020dowhy,tingley2014mediation}). 
% However, the output DAG must be concise to facilitate information elicitation about the validity of the assumptions and communicate the underlying assumptions used for drawing causal inferences. 
However, a main challenge is how to maintain the necessary level of granularity to ensure accurate causal inference. 
The limitations of existing solutions and challenges in constructing the desired C-DAG are discussed, and a limited prototype implementation for solving the CDI problem is presented with preliminary experimental results demonstrating that solving CDI is achievable.}


We further added a discussion about the challenges and opportunities for each one of the system components at each relevant subsection. Please refer to the revised Section \ref{sec:system}.  

Last, we included the following discussion on the system limitations in Section \ref{sec:conc}:


\textsf{We note the following limitations of our proposed CDI system: 
First, the quality of the generated C-DAG may
be affected by factors such as the quality of extracted data
(e.g., incorrect values) and black-box components (e.g., the entity linker used to link values from the input dataset to their corresponding entities in a knowledge graph).
Second, the generated C-DAG may
not be complete, meaning that not all real-life confounding
attributes were observed and extracted, and thus the unconfoundedness assumption is violated. In particular, datasets containing information about people often lack properties about their age or ethnicity, which are common confounding variables. 
Finally, the goal of a CDI is to assist analysts in identifying a correct adjustment set to be controlled for to answer a causal question. While methods for identifying confounding variables through causal DAGs using, for example, backdoor and front-door criteria are well understood, they all rely on the availability of full causal DAGs~\cite{pearl2009causality}. However, in practice, full causal DAGs are often not available~\cite{glymour2019review}. Specifically, in our framework, in which we dynamically integrate data with external sources,
it is not always reasonable to assume that a full causal DAG can be automatically discovered. This is because determining causal relationships oftentimes requires substantial in-domain knowledge.}





\vspace{1mm}
This concludes the summary of the main revisions in the paper.
Below, you will find detailed responses to the reviewers' comments.
Updates made in response to specific comments are highlighted in the revised manuscript using the following colors:
\begin{itemize}
\item \common{Changes mentioned by multiple reviewers in Red}
\item \reva{Reviewer 1 in Blue}
\item \revb{Reviewer 2 in Magenta}
\item \revc{Reviewer 3 in Purple} 
\end{itemize}



\vspace{1mm}
\noindent{\bf REVIEWER 1}

\noindent
\colorbox{pink}{\textbf{W1:}} \emph{It is better for the paper to better introduce the background of causal inference using an example (e.g. a dataset with several attributes that can constitute a graph). The challenges and why data integration can solve the challenges can also be reflected from the example. This will make the paper more convincing.} 

We thank the reviewer for this comment. Please see our response in \colorbox{pink}{\textbf{Point 1}} above. Note the inclusion of Tables \ref{tab:example} and \ref{tab:extracted_att}, Figures \ref{fig:causal_dag} and \ref{fig:c_dag}, and Examples \ref{ex:causal_dag}, \ref{ex:knowledge_extractor}, \ref{ex:data_org}, and \ref{ex:causal_dag_builder}, to help illustrate the challenges of causal inference and how CDI can solve those challenges.


\noindent
\colorbox{pink}{\textbf{W2:}} \emph{As the domain of tabular data is much diverse. Given an arbitrary table, it is in fact hard to discover some tables that can join with it, which may make the solution in this paper impractical.}

We agree with the reviewer on this important issue. In response, we extended the discussion about the limitations of CDI, clarifying this issue. 
We now mention that one of the limitations of CDI is that the generated causal DAG may
not be complete, meaning that not all real-life confounding
attributes were observed and extracted. In particular, datasets containing information about people often lack properties about their age or ethnicity, which are common confounding variables (please see the revised Section \ref{sec:conc}).

We also mention in Section \ref{subsec:knowledgeextraction} that the 
\emph{Knowledge Extractor} faces the challenge of identifying relevant unobserved attributes to be added for any arbitrary input dataset. This can done by the development of dedicated techniques to extract and integrate unobserved confounding variables from different types of external data sources, such as data lakes, knowledge graphs, and unstructured data. Please refer to the revised Section \ref{subsec:knowledgeextraction} for more details. The relevant segment is also reproduced in \colorbox{pink}{\textbf{Point 4}} above.
 
 

\noindent
\colorbox{pink}{\textbf{W3:}} \emph{The paper is to study how data integration can benefit causal inference (help to discover critical confounding variables), and I am also wondering whether causal inference can benefit the DB community, like helping to deduce the root causes of database failures?}

Following the reviewer's suggestion, we have added the following text to Section \ref{sec:intro}: 
 
\textsf{CDI may also be beneficial for the data management community. Causal inference has been shown to be useful for various data management tasks, including query result and classifier explanation \cite{salimi2018bias,alipour2022explaining,youngmann2022explaining}, hypothetical reasoning \cite{galhotra2022hyper}, and ensuring the fairness of predictive models~\cite{zhu2022crab}. However, some of these studies make strong assumptions about the underlying causal DAG that may not hold in practice~\cite{mcnamee2003confounding,henderson2004handbook}. For example, \cite{galhotra2022hyper} assumes that the causal DAG is known, and \cite{salimi2018bias} assumes that all confounding variables are present in the input dataset. To address these issues, a CDI system can be utilized to construct a causal DAG for a given dataset while integrating relevant missing attributes. This not only addresses the limitations of existing studies but also enables the use of causal inference in more complex and realistic scenarios.}

\vspace{2mm}
\noindent{\bf REVIEWER 2}

\noindent
\colorbox{pink}{\textbf{W1:}} \emph{
 Some issues with the manuscript}

Please see our detailed responses to \colorbox{pink}{\textbf{Points D1-D11}} below. 

\noindent
\colorbox{pink}{\textbf{W2:}} \emph{
 In a vision paper, I would have prefered to read less solutions than problems and research directions. }

Following the reviewer's suggestion, we extended the discussion on the system challenges and research opportunities (see our response to \colorbox{pink}{\textbf{Point 4}} above). In return, we narrowed the description of our proposed solutions, which is now only given in Section \ref{sec:poc}. This better distinguishes challenges and proposed solutions.
 

 \noindent
\colorbox{pink}{\textbf{D1:}}\emph{
 I find that this manuscript defines the problem and "rushes" into providing an architecture and preliminary solutions to the problem (especially around the C-DAG-based ones). The issue for the paper is that it reads more like a half-baked research paper, than a vision paper. Section 5.1 could be substantially extended. }

We thank the reviewer for this important comment. As mentioned in the response of \colorbox{pink}{\textbf{Point W2}} above, we have revised Section \ref{sec:system} to point out the challenges a CDI system has to face and corresponding research opportunities. We also moved our solutions description to Section \ref{sec:poc}, the Proof Of Concept Implementation Section. Please refer to the revised Sections \ref{sec:system} and \ref{sec:poc}.
 

  \noindent
\colorbox{pink}{\textbf{D2:}} \emph{
I wonder if it would be worthwhile prividing some more background on DAGs of causal relationships between attributes. Is it always possible to have a DAG? Or do cycles appear when two atteributes are confounding? How do we deal with those? I can think examples of dirty data lakes that containing the same data, but with different names and column formats. For instance, what if two attributes of country (CNTRY: {USA, CHN} vs. Country {United States, China}): won't they have links from one another? Later, in 4.2, I get to read about this exact issue. }

In addition to the changes made in \colorbox{pink}{\textbf{Point 2}}, we revised and extended the text to further clarify the causal DAG concept.
In Section \ref{subsec:data_model}, we revised the text regarding causal DAGs as follows:

\textsf{The input dataset $\mathcal{D}$ contains the exposure ($T$) and outcome ($O$) attributes. 
A \emph{causal DAG} for $\mathcal{D}$ is a DAG whose nodes are
the set of attributes and whose edges capture all causal relationships between the attributes \cite{pearl2000models}. 
% It specifies conditional independencies among the attributes. 
Causal DAGs provide a simple way of graphically representing causal relationships and are particularly helpful in understanding potential sources of bias in causal estimations. It is well-known that such background knowledge is required to determine a causal DAG for a given dataset~\cite{pearl2018book}. A causal DAG can only be as good as the background information used to create it~\cite{pearce2016causal}; a DAG is complete and therefore has a causal interpretation only if it contains all common causes of any two variables. In Section \ref{subsec:dag_builder}, we review existing approaches for building a causal DAG for a given dataset and discuss their limitations.}

We further extended the discussion about the challenges of extracting unobserved confounding attributes, reviewing failure modes that may hinder the ability of a CDI system to build a causal DAG. Specifically, we added the following text to Section \ref{subsec:knowledgeextraction} in line with highlighting challenges and opportunities in each component of the CDI system in \colorbox{pink}{\textbf{Point 4}}:

\textsf{The \emph{Knowledge Extractor} faces the challenge of identifying relevant unobserved attributes to be added for any arbitrary input dataset. The module must operate correctly even in cases of value mismatches, such as when a state name is given explicitly (e.g., Massachusetts) or as a shortcut (e.g., MA). To tackle this challenge, researchers can rely on a rich body of work on entity linking and disambiguation \cite{demartini2013large,lin2020kbpearl,dredze2010entity}.}


As for your specific question about acyclicity, since causes must precede effects, generally, the literature considers causal DAGs rather than causal graphs with cycles \cite{pearl2000models}. That said, feedback loops may appear cyclic. Still, they can be broken down by modeling variables at different times as different variables, modeling a feedback loop without using a cyclic graph. We clarify this point in Section \ref{sec:problem}.

As mentioned by the reviewer, having two attributes that are semantically and distributionally identical is a problem for a CDI system. Such attributes could be unified by the \emph{Knowledge Extractor} in Section \ref{subsec:knowledgeextraction}, pruned by the \emph{Data Organizer} as mentioned in Section \ref{subsec:data_organizer}, or grouped together by the \emph{Causal DAG Builder} as mentioned in our revised Section \ref{subsec:dag_builder}.
% (comment to brit: we should probably mention a sentence or two in the paper itself about the acyclicity constraint. i don't think i even fully understand the reason we have it. pearl just says that he will just focus on these, and that's it. this text can also be shrunk quite a bit, and possibly would need a citation if we add it to the body of the paper


% there are three sources for this acyclicity constraint on the CDI output:
% % statistical assumption for causal inference in many contexts; some demonstrated in cyclic/feedback loop contexts but not thoroughly
% (1) The acyclicity constraint is a commonly required assumption for using background knowledge causal graphs in causal inference tasks like estimation of treatment effects; if CDI system output causal graphs do not hold to this constraint, researchers and analysts would need to make strict, potentially unrealistic assumptions (like all variables are linearly related) to use the causal graph for causal inference.
% % time, causality being directed/asymmetric
% (2) Causality is generally interpreted as an asymmetric relationship; given enough time, some causal systems can be modeled as feedback loops.
% For example, being overweight can prompt frequent hunger pangs; each period of hunger pang thereby prompts patients to eat more to satiate the feeling; as a result, regularly eating more than the patient's baseline would raise their weight further.
% However, an implicit modeling decision in many causal inference contexts is that the time-scale of these changes occurring generally is selected so that the causal contribution is not cyclic. % , in order to adhere to the underlying statistical requirements.
% % https://plato.stanford.edu/entries/causation-probabilistic/ search for '(iii) Asymmetry'
% % https://plato.stanford.edu/entries/causal-models/topics.html look for 'Cycles'
% % cycles and semantically identical items
% (3) Similar to logical and functional dependencies,
% % semantically and distributionally identical attributes will have the property that
% any automatic causal graph construction system will struggle or fail to produce useful output
% % to construct a causal graph if they are
% with semantically and distributionally indistinguishable attributes. Such attributes could be unified by the \emph{Knowledge Extractor} in Section \ref{subsec:knowledgeextraction}, pruned by the \emph{Data Organizer} as mentioned in Section \ref{subsec:data_organizer}, or grouped together by the \emph{Causal DAG Builder} as mentioned in our revised Section \ref{subsec:dag_builder}, reproduced with our response to \colorbox{pink}{\textbf{Point D6}} below.
% (comment to brit: we should probably mention a sentence or two in the paper itself about the acyclicity constraint. i don't think i even fully understand the reason we have it. pearl just says that he will just focus on these, and that's it. this text can also be shrunk quite a bit, and possibly would need a citation if we add it to the body of the paper)
% }

  \noindent
\colorbox{pink}{\textbf{D3:}} \emph{
The related works section could be skipped altogether if the authors could embed those works in the rest of the paper - each on the right spot where background is needed.}

We thank the reviewer for this suggestion. We followed the reviewer's advice in reorganizing the related work references and distributing discussion of related work in the relevant places. 

\noindent
\colorbox{pink}{\textbf{D4:} }
\emph{data integration system is defined by its ability to tie tuples from different sources  --- this is not an entirely true statement. I do understand the intention of the authors, but this refers more to entity resolution and record linking, rather than the (very broad) data integration reseach area. Since this has been used also elsewhere, I'd suggest that the authors rephrase if possible.}

We agree with the reviewer on this important issue. We rephrased the text in Section \ref{sec:intro} as follows: 

\textsf{Distinct from the classical data integration task, where success is defined by its ability
to combine data from different sources and provide users with a unified materialized view of them, the success of a CDI system... } 

  \noindent
\colorbox{pink}{\textbf{D5:}} \emph{
I would love to see a short mention or mapping of classic data integration concepts with causal inference (if the authors believe there is such a connection). For instance, functional dependencies can be seen as a limited form of causal relationship (e.g., Company - CEO if we know the company name we also know the CEO of that company).}

Please refer to our response in \colorbox{pink}{\textbf{Point 2}} above. 

\noindent
\colorbox{pink}{\textbf{D6:}} \emph{
Section 3.1: Is the C-DAG part of the solution, or the problem definition? If it is the former, this part could leave and be moved to further sections. This will separate the problem (which is a large part of the contrubiution of this paper) and the solutions.}

We thank the reviewer for this critical comment.
Indeed, building a C-DAG rather than a full causal DAG is part of our solution and not the problem definition. We have revised the paper accordingly. 


Specifically, in Section \ref{subsec:challenges},
we revised the discussion about the conciseness challenge as follows: 


\textsf{We can potentially extract hundreds of unobserved attributes from given data sources, which can lead to a complex and high-dimensional causal DAG. To overcome this challenge, the CDI system should aim to reduce users' cognitive overhead in interpreting the DAG. It is also crucial to ensure the scalability of causal analysis, as existing tools are not feasible for high-dimensional data~\cite{sharma2020dowhy,tingley2014mediation}.
One approach is to ensure that related attributes are grouped into clusters while still ensuring that the correct set of confounders is identifiable. Thus, a third challenge is to ensure that the output DAG is concise. The CDI system should be able to construct a causal DAG that effectively captures the causal relationships between attributes while maintaining the necessary level of granularity to ensure accurate causal inference. This will enable analysts to efficiently handle high-dimensional data while facilitating information elicitation about the validity of the assumptions used for drawing causal inferences.}

In Section \ref{subsec:dag_builder}, we revised the text as follows: 


\textsf{The desiderata for a desired causal DAG is summarized as follows. First, there is a need to limit the number of nodes in the output DAG. This is critical to ensure that causal analysis is possible for high-dimensional data (which is not feasible for existing tools ~\cite{sharma2020dowhy,tingley2014mediation}) and will reduce analysts' cognitive overhead 
in interpreting the DAG. Second, to ensure the output DAG is comprehensible, only semantically-related attributes (e.g.,} \verb|avg temp|, \verb|snow inch|) \textsf{should be grouped and represented as a single node. Last, we must ensure that the output DAG enables the identification of the right adjustment set of confounders for accurate causal inference. }



\textsf{To address the above desiderata, we propose to build a \emph{cluster causal DAG} (C-DAG)~\cite{anand2022effect}.  
A C-DAG provides only a partial specification of causal relationships among attributes, alleviating the requirement of specifying all causal relationships. In a C-DAG, some attributes are grouped, and only the causal relationships between clusters of attributes are specified. 
Previous work~\cite{anand2022effect}
showed that cause-effect computations can be determined directly from a C-DAG. In the output C-DAG, only semantically-related attributes should be clustered, and the number of nodes should be limited. A remaining open question is how to ensure that the correct adjustment set of confounding attributes is identifiable since, by grouping attributes, we lose information about their inter-relations. We next discuss the main challenges in building a desired C-DAG.}

  \noindent
\colorbox{pink}{\textbf{D8:}} \emph{
In general, problem vs. solutions vs. oportunities/future work could be more clearly distinguishable.}

We agree with the reviewer. As mentioned in \colorbox{pink}{\textbf{Points W2, D1, D6}} above, we moved the description of our initial solutions of the described challenges to Section \ref{sec:poc}, to better distinguish between the challenges and proposed solutions.
%\anna{i don't see it; did we delete it?}


  \noindent
\colorbox{pink}{\textbf{D9:}} \emph{
Could you extend the discussion on robustness a bit more? Is the problem only with missing values? What about the rest of the data quality issues out there?}

Please see our response to \colorbox{pink}{\textbf{Point 3}} above. 



 
  \noindent
\colorbox{pink}{\textbf{D10:}} \emph{
Section 4: "casual analysis tool" => Causal analysis tool}
We thank the reviewer for this comment. We have fixed this typo (and proofread the paper to make sure there are no more typos). 


  \noindent
\colorbox{pink}{\textbf{D11:}} \emph{
"We thus also discard attributes that have functional dependencies with T or O" What is T or O?}

We added a clarification to explain that $T$ is the exposure attribute and $O$ is the outcome in the revised Section \ref{subsec:data_model}. The revision of interest can also be found in \colorbox{pink}{\textbf{Point D2}} as well.


\vspace{2mm}
\noindent{\bf REVIEWER 3}

  \noindent
\colorbox{pink}{\textbf{W1:}} \emph{
The discussion of opportunities and limitations (Sec 5.1) can include more content with enough depth and breadth.}

We thank the reviewer for this comment. We have extended the discussion of future opportunities throughout the paper, identifying research opportunities for each system component. We also included a discussion on the system's limitations in Section \ref{sec:conc}. Please refer to our response to \colorbox{pink}{\textbf{Point 4}} above. 

  \noindent
\colorbox{pink}{\textbf{D1:}}\emph{
I think the main flaw that exists in this vision paper is the discussion of future research opportunities. Based on my personal interpretation, the author only discussed one potential opportunity for each component introduced in the prototype system. I think it would make more sense to propose some more broad discussion corresponding to the challenges identified before (completeness, robustness, and conciseness), which is able to provide more insight into how this new research area could move forward.}

We thank the reviewer for this comment. Please see our response to \colorbox{pink}{\textbf{Point 4}} above. 

  \noindent
\colorbox{pink}{\textbf{D2:}} \emph{
Improve the discussion of opportunities and limitations (Sec 5.1). It could include more content with enough depth and breadth.}


Following the reviewer's advice, we reorganized the discussion about research opportunities throughout the paper. Please see our response to \colorbox{pink}{\textbf{Point 4}} and revised Section \ref{sec:system}.

==> response2.tex <==
\twocolumn

\section*{Response to the Reviewers}
\noindent \textbf{Dear reviewers,}

\noindent 
We would like to reiterate our appreciation to the reviewers for providing us with their valuable feedback, which significantly assisted us in enhancing the quality of our paper.

As a response to the reviewers' feedback, we have included a link to our repository in the paper (please refer to the revised Section \ref{sec:poc}). This repository contains the examined datasets, along with a prototype implementation of our system.




